Faster Robust Tensor Power Method for Arbitrary Order

Tensor decomposition is a fundamental method used in various areas to deal with high-dimensional data. \emph{Tensor power method} (TPM) is one of the widely-used techniques in the decomposition of tensors. This paper presents a novel tensor power method for decomposing arbitrary order tensors, which overcomes limitations of existing approaches that are often restricted to lower-order (less than $3$) tensors or require strong assumptions about the underlying data structure. We apply sketching method, and we are able to achieve the running time of $\widetilde{O}(n^{p-1})$, on the power $p$ and dimension $n$ tensor. We provide a detailed analysis for any $p$-th order tensor, which is never given in previous works.

==> exp_app.tex <==

\section{Additional Experiment Results}

The following sections gather all of our experiment results we collected
to compare our sampling-based robust tensor power method
to a sketching-based robust tensor power method. Our algorithm
has the following parameters to set:

\begin{enumerate}

\item $T$: Number of power iterations
\item $L$: The number of starting vectors of the robust tensor power method
\item $B$: The number of sketches used in sketching, or the number of repetitions of sampling 
\item $b$: The size of the sketch, or the number of indices sampled

\end{enumerate}

In all of our experiments, we fix $T=30$, $L=50$, and change $B$ and $b$
for each input tensor. We observe the squared residual Frobenius norm
to evaluate the performance of each algorithm. We only compute the 
first eigenvalue and eigenvector (rank-1 recovery) of each tensor.
This enables us to run a large collection of tensors within a reasonable time.


 
\subsection{Synthetic tensors with inverse decaying eigenvalues}

The tables shown in this section use synthetic tensors generated with
eigenvalues decaying as $\lambda_i = \frac{1}{i}$. All tensors have rank
$k=100$ and added noise with $\sigma = 0.01$.



\clearpage


 
\subsection{Synthetic tensors with inverse square decaying eigenvalues}

The tables shown in this section use synthetic tensors generated with
eigenvalues decaying as $\lambda_i = \frac{1}{i^2}$. All tensors have rank
$k=100$ and added noise with $\sigma = 0.01$.



\clearpage


 
\subsection{Synthetic tensors with linearly decaying eigenvalues}

The tables shown in this section use synthetic tensors generated with
eigenvalues decaying as $\lambda_i = 1 - \frac{i-1}{k}$. All tensors have rank
$k=100$ and added noise $\sigma = 0.01$.
Due to the slowly decaying eigenvalues, we expect to see large residual
values of rank-1 decomposition, and both algorithms have to work harder to
get a better recovery. Our sampling based method works better especially
when the dimension is large.


\clearpage
\subsection{Results from real-life datasets}


\begin{table}[h]
\begin{center}
    \begin{tabular}{| r | c | c | c | p{6.1cm} |}
    \hline
    {\bf Dataset} & \# {\bf Documents} & \# {\bf Vocabulary} & \# {\bf Words} & {\bf Short Description} \\ \hline
    Wiki & 114274 & 10000 & 58508288 & Wikipedia articles, preprocessed by authors of~\cite{wtsa15} \\ \hline
    Enron~\tablefootnote{ \url{http://www.cs.cmu.edu/~enron/}} & 186501 & 10000 & 16971591 & Enron Email Dataset, preprocessed by authors of~\cite{wtsa15} \\ \hline
    AP~\tablefootnote{ \url{http://www.cs.princeton.edu/~blei/lda-c/}} &2246 & 10473 & 435838 & Associated Press \cite{bnj01}\\ \hline
    NIPS~\tablefootnote{ \label{swz16:uci}\url{https://archive.ics.uci.edu/ml/machine-learning-databases/bag-of-words}} & 1500 & 12419 & 1900000 & NIPS full papers, preprocessed by UCI \\ \hline
    KOS~\tablefootnote{\url{https://archive.ics.uci.edu/ml/machine-learning-databases/bag-of-words}} & 3430 & 6906 & 467714 & KOS blog, preprocessed by UCI \\\hline
    NSF~\tablefootnote{ \url{http://archive.ics.uci.edu/ml/datasets/NSF+Research+Award+Abstracts+1990-2003}} & 49078 & 22170 & 4406190 & NSF research award abstracts 1990-2003 \\ \hline
    \end{tabular}
\end{center}
\caption{List of six real-life datasets}
\label{swz16:tb:datasets}
\end{table}


We used the two same datasets as the
previous work \cite{wtsa15}: Wiki and Enron, as well as four additional
real-life datasets, shown in Table~\ref{swz16:tb:datasets}.  
We use the program from the authors of \cite{tung2015spectral} to build a $K \times
K \times K$ tensor $A _{\mathrm{LDA}}$ for each dataset.  Due to limited time
our experiments only use $K=200$.  We expect to gain more over the
sketching-based method on larger tensors.

Since these tensors comes from real-world applications and are not normalized, 
their Frobenius norm is usually very large.



